Preconditioner Design via the Bregman Divergence

We study a preconditioner for a Hermitian positive definite linear system, which is obtained as the solution of a matrix nearness problem based on the Bregman log determinant divergence. The preconditioner is of the form of a Hermitian positive definite matrix plus a low-rank matrix. For this choice of structure, the generalised eigenvalues of the preconditioned matrix are easily calculated, and we show under which conditions the preconditioner minimises the $\ell_2$ condition number of the preconditioned matrix. We develop practical numerical approximations of the preconditioner based on the randomised singular value decomposition (SVD) and the Nystr\"om approximation and provide corresponding approximation results. Furthermore, we prove that the Nystr\"om approximation is in fact also a matrix approximation in a range-restricted Bregman divergence and establish several connections between this divergence and matrix nearness problems in different measures. Numerical examples are provided to support the theoretical results.

==> _hierarchical.tex <==
\subsection{Block Structured Preconditioner}

The invariance in proposition \ref{prop:bregman_invariance} extends to block diagonal congruence
transformations, extends the application Block matrices are common in large-scale numerical linear algebra. 


\begin{definition}
Let $E_i \in \mathbb{R}^{n_b\times b}$ be the matrix constructed from the identity
of size $n$ by deleting columns $j$ so that $j\notin i$. For $b=1$, $E_i X 
E_j\transp = X_{ij}$. If $X$ is a block matrix ($n_b\geq 2$), then $E_i X 
E_j\transp$ is the $(i,j)^\textnormal{th}$ block of $X$, which we also denote
by $X_{ij}$.
\end{definition}

In practice we cannot invert $A$, or it is as least as hard as the original
problem, so the idea is to impose a certain structure for $X$ that will imply that
we are making some approximations of the corresponding $A$ i.e. replacing by
$\widehat A$. The main idea is to construct a better preconditioner by observing
that in the previous two approaches we have discarded information
on the diagonal. We investigate a preconditioner where we retain
more diagonal dominance, and reduce the rank of the off-diagonal
blocks.\\

For the matrix $S$ of size $n$ we consider an approximant $X$ on the form of a sum of
a block diagonal matrix $D$ (with $n_b$ blocks of size $b$) and a low rank contribution
$K$. This leads to following optimisation problem where $\mathbb{1}$ is the vector 
where all entries are equal to $1$:
\begin{align}
\min_{\substack{D_i\in\Rnbnb\\ K \in Rnn}} &\BregmanLogDet (X, S)\label{min:Bregman:block}\\
\text{s.t.} \; & X = D + \OffDiagonal \circ K\nonumber\\
& D = \blkdiag(D_1,\ldots, D_n),\nonumber\\
& \rank(K) = r.\nonumber
\end{align}

The optimality conditions of \eqref{min:Bregman:block} are given by\footnote{
The optimality conditions of $\BregmanLogDet(X, S\inv)$ are the same, with $S\inv$
replaced by $S$.}:

\begin{subequations}\label{min:Bregman:block:kkt}
\begin{align}
& E_i\transp S\invtransp E_i =  E_i\transp (D + K)\invtransp E_i, \quad 1 \leq i \leq n_b,\label{min:Bregman:block:kkt:D}\\
& E_i\transp (S\inv - (D + K)\inv) E_j = 0, \quad \quad 1 \leq i,j \leq n_b, \quad i\neq j.\label{min:Bregman:block:kkt:K}
\end{align}
\end{subequations}

Imposing further constraints on the structure of $X$ in \eqref{min:Bregman:block:kkt}
leads to different preconditioners.\\

\todo{Lower bounds and minimisers.}

\subsubsection{HODLR Compression}

We say that $X$ is a \emph{hierarchical off-diagonal low rank} (HODLR) matrix
of rank $l$ when either:
\begin{itemize}
\item $X$ is of size at most $2l$,
\item $X$ has the following nested structure:
\[
X = \begin{vmatrix}
X_{11} & X_{12}\\
X_{21} & X_{22}
\end{vmatrix},
\]
where $\rank(X_{12}) \leq l$, $\rank(X_{21}) \leq l$ and the diagonal
matrices are also HODLR of rank $l$.
\end{itemize}

Block matrices are trivially HODLR matrices.

As the following
example shows, using these as approximants in the Bregman divergence
recovers the block Jacobi preconditioner.
\begin{example}
We now give an example of approximating $S\inv$ using the Bregman divergence.
Consider $S$ with $n_b$ blocks $S_{ij}$ of size $b\times b$ and let 
$X = D = \blkdiag(D_1,\ldots, D_n)$. Then \eqref{min:Bregman:block:kkt:D} simplifies to:
\[
E_i\transp S\inv E_i =  E_i\transp D\inv E_i = D_{ii}\inv.
\]
Had we minimised $\BregmanLogDet(X, S\inv)$ instead, this condition would read:
\[
E_i\transp S E_i = S_{ii} = D_{ii}\inv.
\]
Assuming the diagonal blocks $S_{ii}$ are invertible, this leads to a closed
form for $D_{ii}\inv$ thanks to the Woodbury formula, and facilitates parallel
computation.\\

\todo{Does this correspond to Tabeart's work?}
\end{example}

In general, neither $S$ nor $(D + K)\inv$ possess the same structure as $D + K$
and some approximation is necessary. We can recursively traverse the blocks of
$X$

\todo{HODLR approximation: what can be prove? Not sure how much time we
should devote to this.}

\subsubsection{Hierarchical Semiseparable Compression}

Consider the following form of $K$:
\[
K = I_n \otimes Z,
\]
for some $Z\in\Rnbnb$. This means that each off-diagonal block of $S$ is 
approximated by the same $Z$. In this case, $X$ is a \emph{hierarchical
semiseparable} (HSS) matrix. The condition \eqref{min:Bregman:block:kkt:K} now
reads:
\[
\sum_{i\neq j} \transp \big[ (S\inv - (D + K)\inv)\circ\OffDiagonal\big]_{ij} = 0.
\]

\todo{Where do we go from here in practice?}

==> _rubbish.tex <==

\iffalse  % Might want to leave this out until it's more developed/understood.
\begin{remark}
The quantity $\BregmanLogDet(\whS, S)$ is exactly the Itakura-Saito divergence $\Divergence_\textnormal{IS}$ between the vectors $x_n \equiv 1$ and $y_n = 1 + \nu_n$:
\[
\Divergence_\textnormal{IS} (x, y) = \sum_{i=1}^n \frac{x_i}{y_i} - \log  \frac{x_i}{y_i} - 1.
\]
There is also a similarity with the relative entropy. Let $x\inv$ and $y\inv$ denote
sequences where the inverse is taken element-wise. The divergence $\Divergence_\textnormal{Sh}$
associated with the negative Shannon entropy $\psi_\textnormal{Sh}(x) = \sum_{i=1}^n x_i \log x_i -
x_i$ is defined by:
\[
\Divergence_\textnormal{Sh}(x\inv,y\inv) = \sum_{i=1}^n x_i\log\frac{x_i}{y_i\inv} - x_i + y_i\inv.
\]
Note that this quantity is the relative entropy, information divergence, 
or generalised Kullback-Leibler divergence, between $x\inv$ and $y\inv$.\\

To summarise, the nearness $\BregmanLogDet(\whS, S)$ between $\whS$ and $S$ coincides with
the Itakura-Saito divergence between the eigenvalues of its arguments, which for this
problem coincides with the relative entropy between the eigenvalues of their inverses:
\[
\BregmanLogDet(\whS, S) = \Divergence_\textnormal{IS} (\theta, \lambda) = \Divergence_\textnormal{Sh} (\theta\inv, \lambda\inv).
\]
\end{remark}
\fi


\iffalse
We study the Rayleigh quotients $\frac{x\transp S x}{x\transp \tilde S x}$
and $\frac{x\transp S x}{x\transp \whS x}$.

\begin{align*}
\frac{x\transp S x}{x\transp \tilde S x}
& = \frac{x\transp Q(I + Q\inv B Q\invtransp)Q\transp x}{x\transp \whQ(I + \whQ\inv B_r \whQ\invtransp)\whQ\transp x}\\
& = \frac{x\transp Q(I + Q\inv B Q\invtransp)Q\transp x}{x\transp \whQ(I + Q\inv B Q\invtransp)\whQ\transp x}
    \cdot
    \frac{x\transp \whQ(I + Q\inv B Q\invtransp)\whQ\transp x}{x\transp \whQ(I + \whQ\inv B_r \whQ\invtransp)\whQ\transp x}\\
& = \alpha_1 \alpha_2.
\end{align*}

\begin{align*}
\alpha_1
    & = \frac{x\transp Q(I + Q\inv B Q\invtransp)Q\transp x}{x\transp QQ\transp x}
    \cdot\frac{x\transp QQ\transp x}{x\transp \whQ\whQ\transp x}
    \cdot\frac{x\transp \whQ\whQ\transp x}{x\transp \whQ(I + \whQ\inv B \whQ\invtransp)\whQ\transp x}
    = \alpha_1^1 \alpha_1^2 \alpha_1^3.
\end{align*}
\begin{align*}
    \alpha_1^1 \in [1, \frac{\lambda_A + \Lambda_B}{\lambda_A}],\qquad
    \alpha_1^2 \in [\frac{\lambda_A}{\Lambda_\whA}, \frac{\Lambda_A}{\lambda_\whA}],\qquad
    \alpha_1^3 \in [ \frac{\lambda_\whA}{\lambda_\whA + \Lambda_B}, 1],
\end{align*}
so:
\[
\alpha_1 \in [\frac{\lambda_A\lambda_\whA}{\Lambda_\whA(\lambda_\whA + \Lambda_B)}, \frac{(\lambda_A + \Lambda_B)\Lambda_A}{\lambda_A\lambda_\whA}].
\]

\begin{align*}
\alpha_2
    & = \frac{x\transp \whQ(I + Q\inv B Q\invtransp)\whQ\transp x}{x\transp \whQ(I + \whQ\inv B_r \whQ\invtransp)\whQ\transp x}\\
    & = \frac{y\transp(I + Q\inv B Q\invtransp)y}{y\transp(I + \whQ\inv B \whQ\invtransp)y}
    \cdot \frac{y\transp(I + \whQ\inv B \whQ\invtransp)y}{y\transp(I + \whQ\inv B_r \whQ\invtransp)y}\\
    & = \alpha_2^1 \alpha_2^2.
\end{align*}
\begin{align*}
    \alpha_2^1 \in [\frac{\lambda_\whA}{\lambda_\whA + \Lambda_B}, \frac{\lambda_A + \Lambda_B}{\lambda_A}],\qquad
    \alpha_2^2 \in [\frac{\lambda_\whA}{\lambda_\whA + \Lambda_B}, \frac{\lambda_\whA^{r+1} + \lambda_B^{r+1}}{\lambda_\whA^{r+1}}],
\end{align*}
so:
\[
\alpha_2 \in [\frac{\lambda_\whA^2}{(\lambda_\whA + \Lambda_B)^2}, \frac{\lambda_A + \Lambda_B}{\lambda_A}\frac{\lambda_\whA^{r+1} + \lambda_B^{r+1}}{\lambda_\whA^{r+1}}].
\]
In summary,
\begin{lemma}
\[
\frac{x\transp S x}{x\transp \tilde S x} \in [
\frac{\lambda_A\lambda_\whA^3}{\Lambda_\whA(\lambda_\whA + \Lambda_B)^3},
\frac{(\lambda_A + \Lambda_B)^2\Lambda_A}{\lambda_A^2\lambda_\whA}\frac{\lambda_\whA^{r+1} + \lambda_B^{r+1}}{\lambda_\whA^{r+1}}
].
\]
\end{lemma}

Next we do the same for $\frac{x\transp S x}{x\transp \whS x}$:

\begin{align*}
\frac{x\transp S x}{x\transp \whS x} 
& = \frac{x\transp Q(I + Q\inv B Q\invtransp)Q\transp x}{x\transp \whQ(I + G_r)\whQ\transp x}\\
& = \frac{x\transp Q(I + Q\inv B Q\invtransp)Q\transp x}{x\transp \whQ(I + Q\inv B Q\invtransp)\whQ\transp x}
    \cdot
    \frac{x\transp \whQ(I + Q\inv B Q\invtransp)\whQ\transp x}{x\transp \whQ(I + G_r)\whQ\transp x}\\
& = \beta_1 \beta_2.
\end{align*}

$\beta_1=\alpha_1$, so:
\begin{align*}
\beta_2 & = \frac{y\transp (I + Q\inv B Q\invtransp)y}{y\transp (I + \whQ\inv B \whQ\invtransp)y}\cdot \frac{y\transp (I + \whQ\inv B \whQ\invtransp)y}{y\transp (I + G_r) y} = \beta_2^1\beta_2^2.
\end{align*}
\begin{align*}
\beta_2^1 & = \alpha_2^1 \in [\frac{\lambda_\whA}{\lambda_\whA + \Lambda_B}, \frac{\lambda_A + \Lambda_B}{\lambda_A}],\\
\beta_2^2 & \in [\frac{\lambda_\whA}{\lambda_\whA + \Lambda_B}, 1 + \lambda^{r+1}_{\whQ\inv B \whQ\invtransp}],
\end{align*}
so:
\begin{align*}
\beta_2 \in
[\frac{\lambda_\whA^2}{(\lambda_\whA + \Lambda_B)^2},
\frac{(\lambda_A + \Lambda_B)}{\lambda_A} (1 + \lambda^{r+1}_{\whQ\inv B \whQ\invtransp})].
\end{align*}
Thanks to Ostrowski's theorem we have a pessimistic bound on $\lambda^{r+1}_{\whQ\inv B \whQ\invtransp}$, namely
since for all $i$:
\[
\lambda^i_{\whQ\inv B \whQ\invtransp} = \theta^i \lambda_B^i,
\]
$\theta^i \in [\lambda_{\whA\inv},\Lambda_{\whA\inv}]$, then:
\[
\lambda^{r+1}_{\whQ\inv B \whQ\invtransp} \leq  \frac{\lambda_B^{r+1}}{\lambda_\whA}.
\]
So $1 + \lambda^{r+1}_{\whQ\inv B \whQ\invtransp}$ is a larger number than
$\frac{\lambda_\whA^{r+1} + \lambda_B^{r+1}}{\lambda_\whA^{r+1}}$, so a priori
it provides a weaker bound on the spectrum of the preconditioned matrix.
Therefore:

\begin{lemma}
\[
\frac{x\transp S x}{x\transp \whS x} \in 
[\frac{\lambda_A\lambda_\whA^3}{\Lambda_\whA(\lambda_\whA + \Lambda_B)^3},
\frac{(\lambda_A + \Lambda_B)^2\Lambda_A}{\lambda_A^2\lambda_\whA} (\frac{\lambda_\whA + \lambda_B^{r+1}}{\lambda_\whA})
].
\]
\end{lemma}

However, numerically we observe that preconditioning with a scaled matrix is much better in practice. So
we would like to understand how that is. This is either by bounding eigenvalues (does not seem to bear any
fruit), or by looking at clustering of eigenvalues. Ideally we want to show that the eigenvalues of $Q\inv
B_r Q\invtransp$ are more spread out that those of $G_r$.\\

Next we study nearness of the approximations $\tilde S$ and $\whS$:

\begin{align*}
\| S - \tilde S\|
& \leq \| A + B - \widehat A - B_r\|\\
& \leq \| A - \widehat A\| + \| B - B_r\|\\
& = \| A - \widehat A\| + \lambda_B^{r+1}.
\end{align*}
Similarly,

\begin{align*}
\| S - \whS\|
& \leq \| A + B - \widehat A - \whQ G_r \whQ\transp\|\\
& \leq \| A - \widehat A\| + \| \whQ (\whQ\inv B\whQ\invtransp - G_r)\whQ\transp\|\\
& \leq \| A - \widehat A\| + \| \whQ \|^2 \| \whQ\inv B\whQ\invtransp - G_r\|\\
& \leq \| A - \widehat A\| + \| \whQ \|^2  \lambda_{\whQ\inv B\whQ\invtransp}^{r+1}\\
& \leq \| A - \widehat A\| + \| \whQ \|^2  \frac{\lambda_B^{r+1}}{\lambda_\whQ^2}\qquad\textnormal{(Ostrowski)}\\
& = \| A - \widehat A\| +\frac{\Lambda_\whQ^2}{\lambda_\whQ^2} \lambda_B^{r+1}\\
& = \| A - \widehat A\| +\kappa(\whQ)^2 \lambda_B^{r+1}.
\end{align*}

Again, a more pessimistic result than for $\tilde S$.\\
\fi


==> applications.tex <==
\iffalse

\section{Applications}

% https://docs.pymor.org/main/tutorial_lti_systems.html

\subsection{Iterative Methods}


\subsection{Regularised Least Squares}

\fi
